Enforcing Access Control in Virtual Organizations Using Hierarchical Attribute-Based Encryption

Virtual organizations are dynamic, inter-organizational collaborations that involve systems and services belonging to different security domains. Several solutions have been proposed to guarantee the enforcement of the access control policies protecting the information exchanged in a distributed system, but none of them addresses the dynamicity characterizing virtual organizations. In this paper we propose a dynamic hierarchical attribute-based encryption (D-HABE) scheme that allows the institutions in a virtual organization to encrypt information according to an attribute-based policy in such a way that only users with the appropriate attributes can decrypt it. In addition, we introduce a key management scheme that determines which user is entitled to receive which attribute key from which domain authority.

==> conclusions.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}

This paper presents a solution to the problem of distributed policy enforcement in virtual organizations. In particular, it presents a new
dynamic HABE (D-HABE) scheme that addresses the dynamics of these collaborations. Furthermore, the paper makes an important link between
attribute-based encryption schemes and trust management, which is proposed as a mean of determining the attribute keys to be issued in a
virtual organization.

The work presented in this paper suggests some interesting directions for future research.
First of all, the proposed scheme does not address the problem of accountability for key
disclosure. More precisely, a domain authority may create another domain authority at the same level in the hierarchy through the re-randomization of its secret key. In addition, a user may disclose her keys (e.g., by publishing them on the Internet)
without fear of being caught as there is no linkability established between the key and the user.
We are working on improving the scheme to address this problem. In addition, we plan to provide the security proof of the proposed scheme in the standard model where the problem of breaking the
scheme is reduced to a well-studied complexity-theoretic problem.



%The dynamic HABE scheme is a cryptographic scheme for the enforcement of sticky TM policies in dynamic, inter-organizational coalitions of systems (e.g., e-health services).
%Dynamic HABE enhances previously proposed ABE and HABE schemes by enabling principals to encrypt data according to ``abstract'' policies, rather than explicitely specifying the set of principals authorized to access the protected data.
%As a result, data do not need to be re-encrypted as new members join and leave the coalition.
%The scheme, however, restricts this dynamic behavior to coalitions with a hierarchical organizational structure, in which one party coordinates the coalition for its entire lifetime.
%
%A side effect of the scheme is that credentials are released ``per-hierarchy''.
%For instance, officer credentials must be issued by the Dutch Navy for each coalition in which its officers are involved; in fact, the credentials issued within a coalition cannot be used to decrypt documents within another coalition, even if the credential issuer, attribute and subject are the same.
%As future work we plan to increase the dynamicity of the scheme to provide a common solution for the enforcement of sticky policies in both hierarchical and non-hierarchical coalitions of systems (e.g., peer-to-peer systems).
%This would simplify the credential management problem: the same credential (e.g., Dutch officer) could be used to decrypt documents independently from the coalition within which they are issued.
%Therefore, less credentials would be issued and managed by each party.
%
%Furthermore, we plan to investigate techniques to preserve the confidentiality of decryption policies.
%In the current (H)ABE schemes, policies are presented in clear, to allow the requester to know what credentials he has to present to get access to the data.
%However, policies might disclose sensitive information: for example, a policy stating that ``only psychiatrict personnel can access the PHR of a patient'' discloses information about the type of health problems of the patient.
%An interesting approach to this problem is an ``incremental'' disclosure of the policy based on the sensitivity of the credentials required.
%Initially, only less sensitive credentials are requested, as a first protection layer.
%If the requester satisfies these first requirements, he is considered trustworthy enough to see the actual decryption policy.
%A similar approach is discussed in~\cite{MS-VLDB-03}.

%Mention other application domain (e.g, cloud computing) as done in other papers.


==> rw.tex <==
\section{Related Work}
\label{sec:rw}


The concept of identity-based encryption (IBE) was first introduced by Shamir~\cite{shamir1985ibc}. In IBE schemes, the public (i.e.,
encryption) key can be any string, e.g., a user name or email address. The first practical IBE scheme based on bilinear pairing on elliptic
curves was proposed by Boneh and Franklin~\cite{DBLP:journals/siamcomp/BonehF03}. In this scheme, a central domain authority issues private (i.e., decryption) keys to the users based on their identity, using a central master secret key.

Later, several alternative IBE schemes have been proposed. Hierarchical IBE
(HIBE) schemes~\cite{DBLP:conf/asiacrypt/GentryS02,DBLP:conf/eurocrypt/BonehBG05}, for instance, are generalizations of the IBE scheme that
reflect an organizational hierarchy. In HIBE, a domain authority at a certain level in the hierarchy can issue secret keys
only to users and domain authorities at lower levels in the hierarchy. The first HIBE scheme was proposed by Gentry and
Silverberg~\cite{DBLP:conf/asiacrypt/GentryS02}. The security of their scheme is based on the Bilinear Diffie-Hellman (BDH) assumption in
the random oracle model. In~\cite{DBLP:conf/asiacrypt/GentryS02}, the size of ciphertexts and private keys is directly proportional to the
level of a domain authority in the hierarchy. Boneh et al.~\cite{DBLP:conf/eurocrypt/BonehBG05} proposed an alternative HIBE scheme, where
the size of the ciphertext is independent of the hierarchy levels, and the size of the private key is inversely proportional to the level
of a domain authority. However, contrarily to \cite{DBLP:conf/asiacrypt/GentryS02}, the HIBE scheme in
\cite{DBLP:conf/eurocrypt/BonehBG05} requires the depth of the hierarchy to be fixed in the setup phase of the scheme. The scheme in
\cite{DBLP:conf/eurocrypt/BonehBG05} is selective-ID secure in the standard model and fully secure in the random oracle model.

The concept of attribute-based encryption (ABE) was first introduced by Sahai and Waters~\cite{DBLP:conf/eurocrypt/SahaiW05}, though it
was called  fuzzy identity-based encryption by the authors. In their scheme, an identity is represented by a set of attributes. The ABE scheme uses an
attribute space $\Omega$ and a function $F(\omega)$ (called a decryption policy) over a set of attributes $\omega \in \Omega$. A user with
an attribute set $\omega'$ is able to decrypt some encrypted information if $F(\omega')=1$, i.e., if  $\omega'$ satisfies the policy. In ciphertext-policy attribute-based encryption (CP-ABE) schemes~\cite{DBLP:conf/sp/BethencourtSW07,DBLP:conf/ccs/OstrovskySW07}, function
$F$ is associated with the encryption of a message $M$ and a user's secret key is associated with a set of attributes $\omega'\in \Omega$.
In key-policy attribute-based encryption (KP-ABE)~\cite{DBLP:conf/icalp/GoyalJPS08} the idea is reversed, i.e., function $F$ is
associated with a user's secret key, while a message $M$ to be encrypted is associated with an attribute set $\omega'\in \Omega$.

A number of variants of the ABE scheme have been proposed since its introduction. They range from extending its functionality to proposing
schemes with stronger security proofs. For example, the scheme in~\cite{DBLP:conf/secrypt/IbraimiAP10} enables a semi-trusted
entity
to update a decryption policy $F(\omega)$ to a decryption
policy $F(\omega')$ using a re-encryption key provided by the initial encryptor, without allowing the semi-trusted entity to decrypt the information. Recently, Green et al.~\cite{brent-outsourcing} proposed a new ABE scheme which largely reduces the computational
overhead associated with ABE schemes. This is enabled by outsourcing the decryption to a semi-trusted entity by means of a re-encryption
key, similarly to~\cite{DBLP:conf/secrypt/IbraimiAP10}. The semi-trusted entity can then use the re-encryption key to transform the
ciphertext into a constant size El-Gamal style ciphertext. Similarly, in order to improve the performance of ABE schemes, Jin et al.
\cite{DBLP:journals/monet/LiWWR11} propose an ABE scheme that treats attribute hierarchies similarly to traditional role-based access
control. In this scheme, the private key for an attribute at a certain level in the hierarchy can be used to decrypt
a ciphertext associated with attributes at lower levels in the hierarchy. If the attribute hierarchy is not
defined, then the proposed construction can be viewed as a normal ABE scheme.

The work that is closest to the solution proposed in this paper is the one of Wang et al.~\cite{WLW-CCS-10}, which propose a hierarchical
attribute-based encryption (HABE) scheme based on the Gentry and Silverberg's HIBE scheme~\cite{DBLP:conf/asiacrypt/GentryS02}.
In~\cite{WLW-CCS-10}, however, attributes are bound to a specific domain authority during encryption, and hence users with attribute keys issued by
different domain authorities are not able to access the encrypted information. The scheme is therefore not suitable for virtual
organizations, which are the focus of this paper. The next section presents an example of virtual organization in the health-care domain
and shows the limitations of the existing (H)ABE schemes in the proposed scenario.

